Spurious Feature Eraser: Stabilizing Test-Time Adaptation for Vision-Language Foundation Model

Vision-language foundation models have exhibited remarkable success across a multitude of downstream tasks due to their scalability on extensive image-text paired data. However, these models also display significant limitations when applied to downstream tasks, such as fine-grained image classification, as a result of ``decision shortcuts'' that hinder their generalization capabilities. In this work, we find that the CLIP model possesses a rich set of features, encompassing both \textit{desired invariant causal features} and \textit{undesired decision shortcuts}. Moreover, the underperformance of CLIP on downstream tasks originates from its inability to effectively utilize pre-trained features in accordance with specific task requirements. To address this challenge, we propose a simple yet effective method, Spurious Feature Eraser (SEraser), to alleviate the decision shortcuts by erasing the spurious features. Specifically, we introduce a test-time prompt tuning paradigm that optimizes a learnable prompt, thereby compelling the model to exploit invariant features while disregarding decision shortcuts during the inference phase. The proposed method effectively alleviates excessive dependence on potentially misleading spurious information. We conduct comparative analysis of the proposed method against various approaches which validates the significant superiority.

==> sections/back.tex <==
This dual intervention approach is designed to address the nuanced aspects of visual context processing in vision-language models. By manipulating different parts of the image - the background and the main objects - we aim to dissect and understand the model's reliance on various features. The first intervention, focusing on the background, is intended to disrupt the model's habitual reliance on contextual cues that may lead to decision shortcuts. By encouraging predictions with higher entropy in this scenario, we push the model towards a less deterministic, more exploratory stance in contexts typically laden with misleading cues.

Conversely, the second intervention zeroes in on the main objects within the image, aiming to refine the model's focus on essential, task-relevant features. By fostering lower entropy in predictions here, we guide the model towards a more confident, feature-specific approach, where the emphasis is on the salient aspects of the image directly tied to the task at hand.

Through these targeted interventions, we seek to balance the model's approach to image processing - mitigating overreliance on potentially misleading contextual information while sharpening focus on crucial, task-related visual cues. This strategy represents an innovative step in enhancing the adaptability and accuracy of vision-language models, particularly in complex, real-world scenarios where the interplay of various image elements significantly impacts performance.

==> tables/app-errorbar.tex <==
\begin{table*}[ht]
  \centering
    \caption{Zero-shot classification performance for different methods with error bars.}\label{tab:app-errorbar}

{
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{cc|cccccccc}
    \toprule
    \multicolumn{2}{c}{Dataset} & {Vanilla}&MASK  &{TPT} 
    & ROBOSHOT & Alpha-CLIP & {Ours}\\
    \midrule 
    \multirow{3}{*}{Waterbirds}
    &$\text{AVG.}$ &$67.67$ &$71.97$ &$66.88_{0.09}$ &$68.86$ &$67.59$ &$\pmb{78.24_{0.20}}$ \\
    &$\text{W.G.}$  &$40.04$ &$51.53$ &$34.38_{0.21}$ &$52.28$ &$43.15$ &$\pmb{65.25_{0.80}}$\\
    &$\text{GAP}$ &$27.63$ &$20.44$ &$32.50_{0.25}$ &$16.58$ &$24.44$ &${12.99_{0.61}}$\\
    \midrule 

    \multirow{3}{*}{PACS}
    &$\text{AVG.}$ &$91.75$ &$91.45$ &$92.90_{0.07}$ &$92.07$ &$\pmb{93.50}$ &$93.07_{0.05}$\\
    &$\text{W.G.}$  &$59.08$ &$60.71$ &$58.94_{0.53}$ &$66.71$ &$\pmb{73.02}$ &$68.73_{1.18}$ \\
    &$\text{GAP}$ &$32.67$ &$30.74$ &$33.97_{0.46}$ &$25.36$ &${20.48}$ &$24.34_{1.19}$ \\
    \midrule 
     \multirow{3}{*}{CamelDeer}
    &$\text{AVG.}$ &$83.20$ &$93.60$ &$77.67_{1.11}$ &$80.40$ &$92.00$ &$\pmb{95.67_{0.25}}$\\
    &$\text{W.G.}$ &$66.40$ &$87.20$ &$55.33_{2.22}$ &$60.80$ &$84.40$ &$\pmb{91.60_{0.86}}$\\
    &$\text{GAP}$ &$16.80$ &$6.40$ &$22.33_{1.11}$ &$19.60$ &$7.80$ &${4.07_{0.62}}$\\
    \midrule 
    \multirow{3}{*}{SpiderCrab}
    &$\text{AVG.}$ &$66.00$ &$91.40$ &$83.53_{0.41}$ &$73.00$ &$86.20$ &$\pmb{95.33_{0.41}}$ \\
    &$\text{W.G.}$ &$42.00$ &$90.40$ &$72.53_{0.75}$ &$50.40$ &$86.00$ &$\pmb{94.67_{1.05}}$\\
    &$\text{GAP}$ &$24.00$ &$1.00$ &$11.00_{0.49}$ &$22.60$ &${0.20}$ &$0.67_{0.66}$\\

    \bottomrule
    \end{tabular}}}%

   
\end{table*}

==> tables/wosam.tex <==
\begin{table}[ht]
  \centering
  \caption{Zero-shot accuracy performance for Vanilla CLIP and SEraser, where ``w/o Anno.'' indicates the absence of an annotation model like SAM, and the task-irrelevant features are simulated as shown in Fig.~\ref{fig:wosam}.}\label{tab:wosam}
{
  % \resizebox{\columnwidth}{!}{
    \begin{tabular}{cc|cc}
    \toprule
    \multicolumn{2}{c}{Dataset} & {Vanilla}& Ours (w/o Anno.)\\
    \midrule 
    \multirow{2}{*}{Waterbirds}
    &$\text{AVG.}$ &$67.67$ &$72.30_{0.20}$  \\
    &$\text{W.G.}$  &$40.04$ &$48.78_{0.56}$\\
    \midrule 
     \multirow{2}{*}{CamelDeer}
    &$\text{AVG.}$ &$83.20$ &$83.73_{0.09}$ \\
    &$\text{W.G.}$ &$66.40$ &$67.47_{0.19}$ \\ %gap $16.27_{0.09}$
    \midrule 
    \multirow{2}{*}{SpiderCrab}
    &$\text{AVG.}$ &$66.00$ &$77.33_{0.38}$ \\
    &$\text{W.G.}$ &$42.00$ &$64.27_{0.68}$ \\
    \midrule 
  \multirow{2}{*}{PACS} & $\text{AVG.}$ &$91.75$  &$92.21_{0.00}$\\
&$\text{W.G.}$  &$59.08$  &$67.68_{0.11}$ \\
    %gap $13.07_{0.50}$

    \bottomrule
    \end{tabular}}%
\end{table}



